Automating App Review Response Generation Based on Contextual Knowledge

User experience of mobile apps is an essential ingredient that can influence the audience volumes and app revenue. To ensure good user experience and assist app development, several prior studies resort to analysis of app reviews, a type of app repository that directly reflects user opinions about the apps. Accurately responding to the app reviews is one of the ways to relieve user concerns and thus improve user experience. However, the response quality of the existing method relies on the pre-extracted features from other tools, including manually-labelled keywords and predicted review sentiment, which may hinder the generalizability and flexibility of the method. In this paper, we propose a novel end-to-end neural network approach, named CoRe, with the contextual knowledge naturally incorporated and without involving external tools. Specifically, CoRe integrates two types of contextual knowledge in the training corpus, including official app descriptions from app store and responses of the retrieved semantically similar reviews, for enhancing the relevance and accuracy of the generated review responses. Experiments on practical review data show that CoRe can outperform the state-of-the-art method by 11.53% in terms of BLEU-4, an accuracy metric that is widely used to evaluate text generation systems.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> sections/filter.tex <==
\section{Quality Filter Assurance}\label{sec:filter}
We propose a quality filter assurance component to automatically detect the reviews for which the \tool model does not generate good responses. We intend to automatically learn the cases in which the proposed \tool model does not perform well. The poorly-generated responses can be shunt to developers for further inspection before posting. In this section, we introduce the method of the quality filter and the performance of the filter.

\subsection{Quality Assurance Filter}
The proposed quality assurance filter contains three main steps. We first prepare the gold set for filter training. We employ the involved reviews and the corresponding responses generated by \tool in the human evaluation as our gold set. Each review and the corresponding generated message are associated with scores which indicate the extent of accuracy to reply to the review (as shown in Figure \ref{fig:human}). To be conservative, we labeled the reviews that receive the ``\textit{accuracy}'' score of one, two or three from one annotator as ``bad'' and all the other reviews as not ``bad''. Then we extract the unigram tf-idf representations of the reviews as the features, since tf-idf has been widely used in natural language processing for feature representation~\cite{DBLP:journals/tse/FanXLH20,DBLP:conf/kbse/VuNPN15}. 

% We compute the \textit{tf-idf} weight for each keyword in one review as:

% \begin{equation}
%     \text{tf-idf} = \frac{\text{tf}}{\log (\text{df}+1)},
% \end{equation}

% \noindent where $\text{tf}$ and $\text{df}$ of a keyword denote the number of its occurrences in the review and the number of reviews in the dataset containing it, respectively. 
We finally train a Gaussian kernel SVM using stochastic gradient descent (SGD) as the learning algorithm based on the dataset of reviews and their labels. The trained SVM will be adopted to predict whether the \tool model generates a ``bad'' response for a user review.

\subsection{Cross-Validation Evaluation}
We split gold set into 10 folds based on stratified shuffle. For each fold, we train a SVM model on the other 9 folds, and test the SVM model on the one fold. We finally obtained the test results for every fold. Table~\ref{tab:filter} shows the predicts of all the folds. In terms of detecting reviews for which the \tool model will generate ``bad'' responses, the filter has 83.0\% precision and 93.6\% recall. Furthermore, it can reduce 31.8\% of the ``bad'' responses. The results demonstrate the usefulness of the proposed filter assurance component for detecting the poorly-generated responses. Developers can focus on examining the ``bad'' responses during using the proposed \tool model.

\begin{table}[t]
\centering
\caption{Predicted results of the cross evaluation of the quality assurance filter.}\label{tab:filter}
    \scalebox{1.0}{
        \begin{tabular}{c|c| r|r}
        \hline
        \hline
       \multicolumn{2}{c|}{\multirow{2}{*}{Predicted Results}} & \multicolumn{2}{c}{Actual Labels} \\
       \cline{3-4}
       \multicolumn{2}{c|}{}& Not Bad &  Bad \\
         \hline
        \multirow{2}{*}{\begin{tabular}[x]{@{}c@{}}Predicted\\Labels\end{tabular}} & Not Bad & 73 & 15 \\
        & Bad & 5 & 7 \\
        \hline
        \hline
        \end{tabular}
    }
\end{table}
